Automatic Stroke Classification of Tabla Accompaniment in Hindustani Vocal Concert Audio

The tabla is a unique percussion instrument due to the combined harmonic and percussive nature of its timbre, and the contrasting harmonic frequency ranges of its two drums. This allows a tabla player to uniquely emphasize parts of the rhythmic cycle (theka) in order to mark the salient positions. An analysis of the loudness dynamics and timing deviations at various cycle positions is an important part of musicological studies on the expressivity in tabla accompaniment. To achieve this at a corpus-level, and not restrict it to the few recordings that manual annotation can afford, it is helpful to have access to an automatic tabla transcription system. Although a few systems have been built by training models on labeled tabla strokes, the achieved accuracy does not necessarily carry over to unseen instruments. In this article, we report our work towards building an instrument-independent stroke classification system for accompaniment tabla based on the more easily available tabla solo audio tracks. We present acoustic features that capture the distinctive characteristics of tabla strokes and build an automatic system to predict the label as one of a reduced, but musicologically motivated, target set of four stroke categories. To address the lack of sufficient labeled training data, we turn to common data augmentation methods and find the use of pitch-shifting based augmentation to be most promising. We then analyse the important features and highlight the problem of their instrument-dependence while motivating the use of more task-specific data augmentation strategies to improve the diversity of training data.

==> titlepage.tex <==
\begin{titlepage}

\newcommand{\HRule}{\rule{\linewidth}{0.5mm}} % Defines a new command for the horizontal lines, change thickness here

\center % Center everything on the page
 


%----------------------------------------------------------------------------------------
%	TITLE SECTION
%----------------------------------------------------------------------------------------

\HRule \\[0.5cm]
{ \huge \bfseries Structure and Automatic Segmentation of Dhrupad Vocal Bandish Audio}\\[0.5cm] % Title of your document
\HRule \\[1cm]

%----------------------------------------------------------------------------------------
%	HEADING SECTIONS
%----------------------------------------------------------------------------------------

\Large An R\&D project report submitted towards partial fulfillment of the requirements for the degree of \\[.25cm] \textbf{Master of Technology}\\[0.5cm] % Major heading such as course name

%----------------------------------------------------------------------------------------
%	AUTHOR SECTION
%----------------------------------------------------------------------------------------
\Large{ By \\ \vspace{0.5cm} \textbf{M A Rohit\\ % Your name
Roll Number: 183076001}\\
\vspace{1cm}
Under the supervision of:\\ \vspace{0.5cm}
\textbf{Prof. Preeti Rao}}\\ % Supervisor's Name
\vspace{1cm}


%----------------------------------------------------------------------------------------
%	LOGO SECTION
%----------------------------------------------------------------------------------------
\center{\includegraphics[scale=0.15]{figures/logo.png}\\[0.5cm]}
%----------------------------------------------------------------------------------------

\Large{Department of Electrical Engineering\\
Indian Institute of Technology Bombay\\
Mumbai 400076, India\\}
\vspace{1cm}


\Large{May 2020}

\vfill % Fill the rest of the page with whitespace

\end{titlepage}
